Deep Fusion: Capturing Dependencies in Contrastive Learning via Transformer Projection Heads

Contrastive Learning (CL) has emerged as a powerful method for training feature extraction models using unlabeled data. Recent studies suggest that incorporating a linear projection head post-backbone significantly enhances model performance. In this work, we investigate the use of a transformer model as a projection head within the CL framework, aiming to exploit the transformer's capacity for capturing long-range dependencies across embeddings to further improve performance. Our key contributions are fourfold: First, we introduce a novel application of transformers in the projection head role for contrastive learning, marking the first endeavor of its kind. Second, our experiments reveal a compelling "Deep Fusion" phenomenon where the attention mechanism progressively captures the correct relational dependencies among samples from the same class in deeper layers. Third, we provide a theoretical framework that explains and supports this "Deep Fusion" behavior. Finally, we demonstrate through experimental results that our model achieves superior performance compared to the existing approach of using a feed-forward layer.

==> 4.2-experiment_compare.tex <==
\input{4.2.3-Table}
\subsection{Emprical Results on CIFAR10}
\todo[inline]{rewrite based on current results}

In this section, we initiate a detailed empirical comparison, contrasting our methodology with other contemporary advancements focusing on infoNCE loss functions. Throughout the experiments detailed in this section, we adopt SimpCLR \cite{chen2020simple} as our foundational framework for contrastive learning. Specifically, SimpCLR employs a singular backbone network to assess similarities within batch samples. Our backbone model is an 18-layer ResNet, as described in \cite{he2016deep}. The fully-connected layer of ResNet-18 is replaced with a flatten layer to extract embeddings. Subsequently, we train the model using a variety of loss functions to evaluate their performance.

After the training phase, we extract the intermediate outputs (size $512$) from the ResNet backbone. These outputs, functioning as embeddings, are then harnessed to train a 3-layer feed-forward network, having layer widths of $256, 128$, and $64$, respectively. Moreover, we incorporate the use of a Support Vector Machine (SVM) \cite{hearst1998support} and K-Nearest-Neighbor (K-NN), training it with the embeddings generated from the training set, as suggested by \cite{li2020prototypical, yeh2022decoupled}. We then proceed to apply the model for classification tasks on the embeddings derived from the test dataset. 



\input{4.2.1-TFUNSUP}

% \input{4.2.2-TFSUP}

==> 4.2.1-TFUNSUP.tex <==


In this section, our focus is on benchmarking our model against a variety of other self-supervised models, each offering advancements on the infoNCE loss function. For our experiments, we utilize straightforward image augmentations to enhance the training process. These augmentations include 1) Random Crop, with a scale range of $(0.8, 1)$, and 2) Color Jitter, characterized by settings of $\text{brightness}=0.2, \text{contrast}=0.2, \text{saturation}=0.2, \text{hue}=0.1$. Following the initial phase of contrastive learning, we fine-tune a final 3-layer Feed-Forward Network (FFN) using the entire label set. This step primarily aims to explore the maximum potential performance that each loss function can achieve.

The loss functions selected for this comparative study include the InfoNCE \cite{oord2018representation}, Decoupled Contrastive Learning loss (DCL) \cite{yeh2022decoupled}, BarlowTwins \cite{zbontar2021barlow}.
%, and Variance-Invariance-Covariance Regularization (VICreg) \cite{bardes2021vicreg}
To ensure a level playing field, a 1-layer TransFusion model serves as our standard benchmark to avoid the confounding effects of additional learnable parameters. Nevertheless, we also report the peak results from a more complex 9-layer TransFusion model. Both variations construct weight matrices $\W_Q, \W_K, \W_V \in \bR^{512 \times 512}$. The 1-layer TransFusion model introduces fewer than 0.5M parameters, while the 9-layer model adds an additional 7M parameters.

The results, as summarized in Table \ref{unsup-CIFAR10-table}, highlight the competitive edge of the TransFusion approach in the self-supervised learning landscape. The 1-layer TransFusion model not only surpasses its contemporaries in performance but does so with a minimal increase in computational time. This efficacy is even more pronounced in the 9-layer TransFusion model, which achieves the highest overall performance in the comparison. Notably, these improvements in performance are attained without a proportional increase in training time.


==> 4.2.2-TFSUP.tex <==

\subsubsection{Supervised Learning}
In this section, we compare our approach with the Supervised Contrastive Learning method referred to as \textit{SupCon} \cite{khosla2020supervised}.
\textit{SupCon} essentially represents a modified variant of \textit{InfoNCE}, but with the incorporation of supervised labels. This implies that, within each batch, images belonging to the same class are expected to exhibit high similarity, while those from different classes should display minimal similarity.
Our backbone for both methods are pre-trained on the ImageNet1K dataset. 

For this experiment, we did not introduce any augmentation techniques. To enhance training performance, the input images were resized from dimensions of $(32, 32, 3)$ to $(224, 224, 3)$. 
The results in Table \ref{CIFAR10-table} clearly indicate that \textit{TransFusion} consistently outperforms \textit{SupCon}, even when \textit{SupCon} is trained with a larger batch size—a practice commonly thought to be more effective for contrastive learning, as noted in \cite{chen2020simple}. Remarkably, \textit{ResNet18} achieves an accuracy of $0.935$ when trained with full labels using cross-entropy loss in our own experiment. This underscores that 1-layer \textit{TransFusion} achieves even better performance to a fully-supervised model.



==> 4.2.3-Table.tex <==

\begin{table*}
\setlength{\tabcolsep}{5pt}
\centering
\begin{tabular}{l|c|cccc|c}
\hline
Model       & Batch Size  & 3-FFN & SVM & K-NN (k=50) & K-NN (k=200) & Time (min) \\
\hline
InfoNCE      & 128               &	0.3854 & 0.3728 &	0.3398& 	0.32    & 990      \\
DCL & 128 & 0.3736 & 0.383 & 0.3099 & 0.2962 & 705\\
BarlowTwins & 128 & 0.4827 & 0.5032 & \textbf{0.4259} & 0.4085 & 752\\
\textbf{TransFusion 1-Layer} & 128                & \textbf{0.5231} &\textbf{0.5102}  & 0.4231 &   \textbf{0.4107}     & 764       \\ \hline
\textbf{TransFusion 9-Layer} & 128                &\textbf{0.5626} &  \textbf{0.5430}	&	\textbf{0.4616} & 	\textbf{0.4453}	& 706      \\ \hline
\end{tabular}
\caption{Self-Supervised classification accuracy (0-1) for CIFAR-10 Using SimpCLR with different loss functions. Each model was trained with ResNet18 as the underlying architecture, underwent a 200-epoch training process, and fined-tuned with $100\%$ labels.}
\label{unsup-CIFAR10-table}
\end{table*}

% \begin{table*}[h]
% \setlength{\tabcolsep}{5pt}
% \centering
% \begin{tabular}{l|c|cccc|c}
% \hline
% Model       & Batch Size  & 3-FFN & SVM & K-NN (k=50) & K-NN (k=200) & Time (min) \\
% \hline
% SupCon      & 128               &0.8121   & 0.8049       & 0.7907      & 0.7717       & 352           \\
% SupCon      & 1024               & 0.9091 & 0.9056       & 0.9002      & 0.8931       & 641           \\
% \textbf{TransFusion 1-Layer} & 128                & \textbf{0.9475} & \textbf{0.9309}       & \textbf{0.9355}      & \textbf{0.9350}       & 368       \\ \hline
% \textbf{TransFusion 9-Layer} & 128                & \textbf{0.9489} &	\textbf{0.9432}	   & \textbf{0.9487}      & \textbf{0.9487}       & 380       \\ \hline \hline
% ResNet-18 & 128 & 0.935   & - & - & - & - \\
% \hline
% \end{tabular}
% \caption{Fully-Supervised classification accuracy (0-1) for CIFAR-10 Using SimpCLR with different loss functions. Each model was trained with ResNet18 as the underlying architecture and underwent a 200-epoch training process.}
% \label{CIFAR10-table}
% \end{table*}


==> Old-1-model.tex <==

\section{TransFusion} 
\todo[inline]{Model and Loss function need justification. Under what circumstances TransFusion is better than MLP?}
\todo[inline]{Less modification from Transformer is better.}
\label{sec-model}



\todo[inline]{How does TransFusion better than MLP as the projector?}

In this section, we present our primary contribution: \textit{TransFusion}. Initially, we provide a mathematical definition of the model and elucidate the underlying principles of the fusion process. Subsequently, we describe the custom-tailored loss function employed in \textit{TransFusion}, which is optimized to enhance the effects of contrastive learning.
The fundamental objective of \textit{TransFusion}, akin to other contrastive learning models, is to generate embeddings that proficiently differentiate between various classes. This entails that samples from the same class should exhibit closer proximity in the embedding space in comparison to those from disparate classes.


\subsection{Model}
To achieve this goal, \textit{TransFusion} takes a batch of input samples and generates a non-negative affinity matrix, which reflects the similarities between pairs of samples. Higher values in the affinity matrix at the $i,j$'th entry indicate stronger similarities between sample $i$ and sample $j$. The model is then trained by minimizing the Jensen-Shannon Divergence (JSD; more on this choice below) between the output affinity matrix and a target affinity matrix, which denotes as $\Y \in \{0,1\}^{n \times n}$:
\begin{align}
    [\Y]_{ij} = \begin{cases} 1  & i,j\text{ in the same class and } i \neq j, \\
    %\varepsilon^\tau & i,j\text{ in the same parent class but $\tau$ depths away} \\
    0 & \text{otherwise.}
    \end{cases}
    \label{Y_def}
\end{align}
\textit{TransFusion} adeptly manages two distinct scenarios: (i) the unsupervised case, wherein affinity is determined through data augmentation, and (ii) the supervised case, where affinity is established based on class labels.


Similar to Transformer, \textit{TransFusion} also consists of identical TransFusion blocks. 
Denote the input matrix as $\X \in \mathbb{R}^{n \times m}$, where $m$ represents the ambient dimension, and $n$ represents the batch size. Furthermore, if we denote $\X^\ell$ as the input of the $\ell$'th \textit{TransFusion} block, then $\ell$'th block can be defined as:
\begin{align}
    &\A^{\ell} := (\X^{\ell}\W_Q^{\ell})(\X^{\ell}\W_K^{\ell})^\top, \label{eq:affinity}\\
    &\X^{\ell + 1} := \text{ReLu}(\A^\ell) (\X^{\ell}\W_V^\ell) + \X^{\ell},
    \label{eq:embedding}
\end{align}
where $\W_Q^\ell$, $\W_K^\ell$, and $\W_V^\ell \in \mathbb{R}^{m \times m}$ represent the learn-able parameters. For training stability and subsequent analysis, $\mathbf{X}^\ell$ are normalized before every block $\ell$ so that each entry has unit length.
The output of the \textit{TransFusion} is the last block's affinity matrix $\mathbf{A}^{d}$, where $d$ is the number of blocks in the \textit{TransFusion}.

To gain deeper insight into the \textit{TransFusion} model's functioning, let us delve into the three key components: queries $\X\W_Q$, keys $\X\W_K$, and values $\X\W_V$. The output of each block is obtained by calculating cosine-similarity queries and keys, and then aggregating a similarity-weighted sum of the values.
Under this mechanism, if the model learns an effective linear transformation of queries and keys, the similarity between samples from the same class can be high, whereas the similarity from the different class can be low. Using this as the weight in the next weighted-sum calculation, samples from the same class shall be able to fuse closer to each other (as demonstrated in Figure \ref{diagram}). 
To further leverage this fusion effect, we change the softmax function in the original attention block to elemental-wise ReLU, which gives us important advantages:
\begin{itemize}
    \item Increased clustering flexibility: 
    By adopting elementalwise ReLU, multiple elements with high similarity scores can fuse into the same cluster. This approach facilitates the integration of a broader range of elements into clusters.
    \item Enhanced model non-linearity: It is important to note that the model does not necessarily require a feed-forward layer immediately after each attention block. However, by incorporating an activation function at this stage, we introduce non-linearity into the model, thereby fortifying its resilience and adaptability.
\end{itemize}

\subsection{Loss Function}
Our training objective is to minimize the Jensen-Shannon divergence between the last block's affinity matrix $\mathbf{A}^{d}$ and the target affinity matrix $\mathbf{Y}$:
\begin{align}
\L_{\text{TF}}(\mathbf{A}^{d}, \Y) := \sum_{i,j} [\Y]_{i,j} \frac{[\Y]_{i,j}}{ g([\mathbf{A}^{d}]_{i,j})/2 + [\Y]_{i,j}/2 }
+ \sum_{i,j} [\mathbf{A}^{d}]_{i,j} \frac{[\mathbf{A}^{d}]_{i,j}}{ g([\mathbf{A}^{d}]_{i,j})/2 + [\Y]_{i,j}/2 }\label{L_TF}
\end{align}
where $g(\cdot)$ is a normalizing function that converts real numbers into probabilities, specified as:
\begin{align}
    g(\mathbf{A}^{d}) := \text{Row-Normalize}((\mathbf{A}^{d})^2)
    \label{g_def}
\end{align}

Remarkably, if we use \textit{Kullback-Leibler Divergence} \cite{kullback1951information} instead, and set $g(\cdot)$ to be the row-wise \textit{Softmax}, our loss with a one-layer \textit{TransFusion} model behaves identically to \textit{InfoNCE} and \textit{SupCon}. The detailed proof is available in Appendix \ref{Appendix: InfoNCE}. The reasoning behind our choice of loss is based on the following considerations:
\begin{itemize}
    \item \textit{KL-Divergence}'s inherent asymmetry becomes particularly problematic the context where a majority of entries in $\Y$ are filled with zeros. To see this, take any pair of samples $i$ and $j$ belonging to different classes, the loss term $\left([\Y]_{i,j} \log \frac{[\Y]_{i,j}}{[g(\A)]_{i,j}}\right)$ prevents the model from penalizing the positive value of the affinity term $[g(\A)]_{i,j}$ as the target affinity is zero, i.e. $[\Y]_{i,j} = 0$. Although the normalization within $g$ might indirectly influence $[g(\A)]_{i,j}$ to be small, this effect is relatively minor compared to the influence other terms. In simpler terms, this loss function strongly encourages embeddings from the same class to be close to each other while largely disregarding the distances between embeddings from different classes. \textit{Jensen-Shannon Divergence}, on the other hand, is a symmetric loss that avoids singularity with target affinities being zero. 

    \item \textit{Softmax} converts negative values to low probability. However, in our unique context, such negativity does not necessarily signify insignificance. To illustrate, consider the case two embedding vectors $\z_i, \z_j$ lies in the same linear subspace, we can ensure that the magnitude of the affinity is large, possibly equal to $||\z_i||_2||\z_j||_2$. However, we cannot tell whether two vectors face the same direction or exact opposite directions. This latter scenario results in a negative projection value. If negative values are converted to low probabilities, as done by \textit{Softmax}, it can limit the model's ability to effectively discern and utilize the underlying substructures within the embedding space. To address this, we square the entries in the affinity matrix. By doing so, we treat both negative and positive affinities equally, allowing for a more flexible and effective use of the embedding space.
\end{itemize}


Through our ablation studies (Appendix \ref{softmaxEmpirical}), we have uncovered an enhancement in stability of our custom loss function \eqref{L_TF} and \eqref{g_def} in comparison to alternative choices, including \textit{InfoNCE}. This improvement is evident in both performance and resilience to changes in the learning rate.


% The rationale behind this choice lies in the potential existence of negative affinity scores within $\A$, a scenario where traditional \textit{Softmax} treatment might designate negative values as indicative of "low probability." However, in our unique context, such negativity does not necessarily signify insignificance.
%     To illustrate, consider the case where Query $\q_i$ perfectly captures the subspace of Key $\k_j$. We can ensure that the magnitude of the projection from $\q_i$ to $\k_j$ is large, possibly equal to $||\q_i||_2$. However, we cannot tell whether two vectors face the same direction or exact opposite directions. This latter scenario results in a negative projection value. Consequently, the act of converting negative values to low probabilities inadvertently constricts the model's capacity to flexibly capture the intrinsic substructure of the Keys.







%where $\varepsilon$ is a decay constant. An example can be referred to Figure \ref{affinity}. 

%\begin{figure}
%\centering
%\includegraphics[trim=4.5cm 4.8cm 4cm 3.2cm, clip=true, width=0.45\textwidth]{graphs/structuralAffinity.pdf}
%\caption{Contract Affinity matrix $\Y$ based on the hierarchical structure of the data. Black pixel in the affinity matrix represents 1, and gray pixel represents $\varepsilon$.}
%\label{affinity}
%\end{figure}

% To attain our objective, one viable approach is to minimize the \textit{Kullback-Leibler Divergence} \cite{kullback1951information} between $\Y$ and $g(\A)$, where $g:\mathbb{R}^{n \times n} \to \mathbb{R}^{n \times n}$ represents a function that transforms affinities into probabilities.

% However, there is a significant concern with the use of \textit{KL-Divergence} due to its inherent asymmetry. This issue becomes particularly problematic in this context, as a majority of entries in $\Y$ are filled with zeros. To see this, take any pair of samples $i$ and $j$ belonging to different classes, the loss term $\left([\Y]_{i,j} \log \frac{[\Y]_{i,j}}{[g(\A)]_{i,j}}\right)$ prevents the model from penalizing the positive value of the affinity term $[g(\A)]_{i,j}$ as the target affinity is zero, i.e. $[\Y]_{i,j} = 0$. Although the normalization within $g$ might indirectly influence $[g(\A)]_{i,j}$ to be small, this effect is relatively minor compared to the influence other terms. In simpler terms, this loss function strongly encourages embeddings from the same class to be close to each other while largely disregarding the distances between embeddings from different classes.

% To solve this issue, we use \textit{Jensen-Shannon Divergence} , which is a symmetric loss that avoids singularity with entries being zero. Specifically,
% \begin{align}
% \L_{\text{TF}}:= \D(\Y || g(\A)/2 + \Y/2) + \D(g(\A) || g(\A)/2 + \Y/2) \label{L_TF}
% \end{align}
% where $\D$ denotes \textit{KL-Divergence} loss. As for the selection of $g(\A)$, we deliberately opt for using row-normalized of $\A^2$, i.e.
% \begin{align}
%     g(\A) := \text{Row-Normalize}(\A^2)
%     \label{g_def}
% \end{align}








